Paraphrase Generation with Latent Bag of Words

Paraphrase generation is a longstanding important problem in natural language processing. In addition, recent progress in deep generative models has shown promising results on discrete latent variables for text generation. Inspired by variational autoencoders with discrete latent structures, in this work, we propose a latent bag of words (BOW) model for paraphrase generation. We ground the semantics of a discrete latent variable by the BOW from the target sentences. We use this latent variable to build a fully differentiable content planning and surface realization model. Specifically, we use source words to predict their neighbors and model the target BOW with a mixture of softmax. We use Gumbel top-k reparameterization to perform differentiable subset sampling from the predicted BOW distribution. We retrieve the sampled word embeddings and use them to augment the decoder and guide its generation search space. Our latent BOW model not only enhances the decoder, but also exhibits clear interpretability. We show the model interpretability with regard to \emph{(i)} unsupervised learning of word neighbors \emph{(ii)} the step-by-step generation procedure. Extensive experiments demonstrate the transparent and effective generation process of this model.\footnote{Our code can be found at \url{https://github.com/FranxYao/dgm_latent_bow}}

==> img/sec_model.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\textwidth]{img/model.png}
\caption{\label{fig:model} Our model equip the seq2seq model(lower part) with latent bag of words(upper part). 
% \noteJPC{this is a silly comment but this figure would be much more clear if you put some colored boxes separating seq2seq from LBOW.  try that? boxes that are behind the text, with rounded corners, that have some white horizontal space separating them, and use some nice qualitative colorbrewer2 colors?}
}
\end{figure}

\section{Model}
\label{sec:model}
Our goal is to extend the seq2seq model (figure \ref{fig:model} lower part) with differentiable content planning and surface realization (figure \ref{fig:model} upper part). 
We begin with a discussion about the seq2seq base model. 

\subsection{The Sequence to Sequence Base Model.} 
\label{ssec:enc_dec_base}

The classical seq2seq model encodes the source sequence $x = x_1, x_2, ..., x_m$ into a code $h$, and decodes it to the target sequence $y$ (Figure~\ref{fig:model} lower part), where $m$ and $n$ are the length of the source and the target, respectively \citep{Sutskever2014SequenceTS, Bahdanau2015NeuralMT}. 
% \noteJPC{include some basics, like the reference, and the fact that $enc_\phi$ is a deep network (typically an LSTM or BiLSTM), and so on.  Also mention how it is trained} 
The encoder enc$_{\psi}$ and the decoder dec$_\theta$ are both deep networks. 
In our work, they are implemented as LSTMs\citep{hochreiter1997long}. 
The loss function is the negative log likelihood.
%
\begin{equation} \label{eq:enc_dec_base}
\begin{split}
    h &= \text{enc}_{\psi}(x) \\
    p(y| x) &= \text{dec}_\theta(h) \\ 
    \mathcal{L}_{\text{S2S}} &= \mathbb{E}_{(x^{\star},y^{\star}) \sim \mathbb{P}^\star} [- \log p_\theta(y^{\star} | x^{\star})],
\end{split}
\end{equation}
%
where $\mathbb{P}^\star$ is the true data distribution.
The model is trained with gradient based optimizer, and we use Adam \citep{kingma2014adam} in this work. 
In this setting, the code $h$ does not have direct interpretability. 
% To add interpretability, the variational autoencoding framework \citep{kingma2013auto} models its code  to be from certain families like Gaussian. 
% \noteJPC{is that really what Kingma2013 does? }
% This gives the latent code a statistical interpretability 
% \noteJPC{this point needs work... I don't really know what it means}. 
% However, intuitively, discrete latent variables might be a better fit to the discrete nature of text.
% It is also easier to ground discrete variables with linguistic interpretability.
To add interpretability, in our model, we ground the meaning of a latent structure with lexical semantics. 
% \noteJPC{notice that this is the first time you say lexical.  So it comes out of the blue and is confusing.  I was expecting a point about interpretability...}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Bag of Words for Content Planning.}
\label{ssec:hierarchical_latent}
% For sequence generation tasks, bag-of-words (BOW) \noteJPC{cite?} can be seen as a straightforward model interpretation \noteJPC{interpretation of what?}.   
Now we consider formulating a plan as a bag of words before the surface realization process.
Formally, let $\mathcal{V}$ be the vocabulary of size $V$; then a bag of words (BOW) $z$ of size $k$ is a \textit{random set} formulated as a $k$-hot vector in $\mathbb{R}^V$. 
We assume $z$ is sampled from a base categorical distribution $p(\tilde{z} | x)$ by $k$ times without replacement.  
Directly modeling the distribution of $z$ is hard due to the combinatorial complexity, so instead we model its base categorical distribution $p(\tilde{z} | x)$. 
In paraphrase generation datasets, one source sentence may correspond to multiple target sentences.  
Our key modeling assumption is that the BOW from target sentences (target BOW) should be similar to the neighbors of the words in the source sentence. 
As such, we define the base categorial variable $\tilde{z}$ as the mixture of all neighbors of all source words. Namely, first, for each source word $x_i$, we model its neighbor word with a one-hot $z_{ij} \in \mathbb{R}^V $ : 
%
\begin{equation} \label{eq:discrete_neighbor}
    p(z_{ij} | x_i) = \text{Categorical}(\phi_{ij}(x_i)) 
\end{equation}
%
The support of $z_{ij}$ is also the word vocabulary  $\mathcal{V}$ and $\phi_{ij}$ is parameterized by a neural network. 
In practice, this can be implemented by a softmax layer on top of the output of each timesteps from the encoder LSTM.
We assume a fixed total number of neighbors $l$ for each $x_i$ ($j = 1, ..., l$).
We then mix the probabilities of these neighbors: %, forming a mixture of categorical (or mixture of softmax) random variables: 
%
\begin{equation} \label{eq:neighbor_mixture}
    \tilde{z} \sim p_{\phi}(\tilde{z} | x) = \frac{1}{ml}\sum_{i, j} p(z_{ij} | x_i)
\end{equation}
%
where $ml$ is the maximum number of predicted words.
$\tilde{z}$ is a categorical variable mixing all neighbor words.  % distributions of each source words.
We construct the bag of words $z$ by sampling from $p_{\phi}(\tilde{z} | x)$ by $k$ times without replacement. 
Then we use $z$ as the plan for decoding $y$. 
The generative process can be written as: 
%
\begin{equation} \label{eq:generative}
  \begin{split}
  z &\sim p_{\phi}(\tilde{z} | x) \quad \text{(sample $k$ times without replacement)} \\
  y &\sim p_\theta(y | x, z) = \text{dec}_\theta(x, z) 
  \end{split}
\end{equation}
%
For optimization, we maximize the negative log likelihood of $p(y | x, z)$ and $p_{\tilde{z}}(\tilde{z} | x)$: 
%
\begin{equation} \label{eq:optimization}
\begin{split}
    \mathcal{L}_{\text{S2S}'} &= \mathbb{E}_{(x^{\star},y^{\star}) \sim \mathbb{P}^\star, z \sim p_\phi(\tilde{z} | x)} [- \log p_\theta(y^{\star} | x^{\star}, z)] \\  
    \mathcal{L}_{\text{BOW}} &= \mathbb{E}_{z^* \sim \mathbb{P}^*} [- \log p_{\phi}(z^*|x)] \\  
    \mathcal{L}_{\text{tot}}  &= \mathcal{L}_{\text{S2S}'}  + \mathcal{L}_{\text{BOW}} 
\end{split}
\end{equation}
% 
where $\mathbb{P}^*$ is the true distribution of the BOW from the target sentences. 
$z^*$ is a $k$-hot vector representing the target bag of words.\footnote{One could also view $\mathcal{L}_{\text{BOW}}$ as a regularization of $p_\phi$ using the weak supervision from target bag of words. Another choice is to view $z$ as completely latent and infer them like a canonical latent variable model. We find out using the target BOW regularization significantly improves the performance and interpretability.}
$\mathcal{L}_{\text{tot}}$ is the total loss to optimize over the parameters $\psi, \theta, \phi$. \footnote{One could also consider variational inference (VI) with $q(z|x)$ and regularize the variational posterior. We find out directlg optimizing the likelihood is sufficent so we leave VI as future work.} 
Note that for a given source word in a particular training instance,
% for the neighbor distribution $z_i$ of a particular word $x_i$, 
the NLL loss does not penalize the predictions not included in the targets of this instance.
This property makes the model be able to learn different neighbors from different data points, i.e., the learned neighbors will be at a corpus level, rather than sentence level. 
We will further demonstrate this property in our experiments. 

\subsection{Differentiable Subset Sampling with Gumbel Top-k Reparameterization.}
\label{ssec:gumbel_topk}
% $\mathbb{P}_z$ models all words in all target sentences.
% To formulate a generation plan, since not all target words are required to build a sentence, one option is to directly extract its $k$ most probable words ($k < ml$) as the plan.
% Then we retrieve the corresponding word embeddings from the embedding table, re-weight them with $\mathbb{P}_z$, and use the weight average of them to be the initial state of the decoder LSTM. 
% Alternatively, to inject randomness into the model, we consider sampling $k$ words from $\mathbb{P}_z$.
% This will require the reparameterization trick for sampling a subset from a discrete distribution.

As is discussed in the previous section, the sampling of $z$ (sample k items from a categorical distribution) is non-differentiable. 
\footnote{One choice could be the score function estimator, but empirically it suffers from high variance. }
To back-propagate the gradients through $\phi$ in $\mathcal{L}_{\text{S2S}'}$ in equation \ref{eq:optimization}, we choose a reparametrized gradient estimator, which relies on the gumbel-softmax trick.
Specifically, we perform differentiable subset sampling with the 
gumbel-topk reparametrization \citep{Kool19GumbelTopK}. Let the probability of $\tilde{z}$ to be $\pi_1, ..., \pi_{\mathcal{V}}$, we obtain the perturbed weights and probabilities by: 
%
\begin{equation} \label{eq:gumbel_topk}
\begin{split}
    a_i &= \log \pi_i + g_i \\ 
    g_i &\sim \text{Gumbel}(0, 1) \\
    \pi_i' &= \frac{\exp{a_i}}{\sum_i \exp(a_i)}
\end{split}
\end{equation}
%
Retrieving the $k$ largest weights topk$(a_1, ..., a_\mathcal{V})$ will give us $k$ sample \textit{without replacement}.
This process is shown in dashed lines in figure \ref{fig:model}. 
We retrieve the $k$ sampled word embeddings $w_1, ..., w_k$ and re-weight them with the gumbel-pertrubed probability $\pi_i'$.
Then we used the average of the weighted word embeddings as the decoder LSTM's initial state to perform surface realization.

Intuitively, in addition to the sentence code $h$, the decoder also takes the weighted sample word embeddings and performs attention\citep{Bahdanau2015NeuralMT} to them; thus differentiability is achieved. 
This generated plan will restrict the decoding space towards the bag of words of the target sentences. 
More detailed information about the network architecture and the parameters are in the appendix.
In section \ref{sec:experiments}, we use extensive experiments to demonstrate the effectiveness of our model. 

